EVOQUER: Enhancing Temporal Grounding with Video-Pivoted BackQuery Generation

Temporal grounding aims to predict a time interval of a video clip corresponding to a natural language query input. In this work, we present EVOQUER, a temporal grounding framework incorporating an existing text-to-video grounding model and a video-assisted query generation network. Given a query and an untrimmed video, the temporal grounding model predicts the target interval, and the predicted video clip is fed into a video translation task by generating a simplified version of the input query. EVOQUER forms closed-loop learning by incorporating loss functions from both temporal grounding and query generation serving as feedback. Our experiments on two widely used datasets, Charades-STA and ActivityNet, show that EVOQUER achieves promising improvements by 1.05 and 1.31 at R@0.7. We also discuss how the query generation task could facilitate error analysis by explaining temporal grounding model behavior.

==> dataset.tex <==
\section{Dataset} 
%0.25 PAGE 
\citet{krishna2017dense} presents ActivityNet Captions Dataset. 

ActivityNet dataset is presented in~\cite{krishna2017dense}. 

\subsection{Charades}
This data set, collected through Amazon Mechanical Turk, is comprised of 9,848 roughly 30 second videos of daily human activities. Similar to a game of charades, each video corresponds to a set of annotated actions and objects from a fixed set of vocabulary. 27,847 textual descriptions are provided for the videos with text queries having a maximum length of 10. \citet{sigurdsson2018charades} 

\subsection{ActivityNet}
